Estimating Leaf Water Content using Remotely Sensed Hyperspectral Data

Plant water stress may occur due to the limited availability of water to the roots/soil or due to increased transpiration. These factors adversely affect plant physiology and photosynthetic ability to the extent that it has been shown to have inhibitory effects in both growth and yield [18]. Early identification of plant water stress status enables suitable corrective measures to be applied to obtain the expected crop yield. Further, improving crop yield through precision agriculture methods is a key component of climate policy and the UN sustainable development goals [1]. Leaf water content (LWC) is a measure that can be used to estimate water content and identify stressed plants. LWC during the early crop growth stages is an important indicator of plant productivity and yield. The effect of water stress can be instantaneous [15], affecting gaseous exchange or long-term, significantly reducing [9, 18, 22]. It is thus necessary to identify potential plant water stress during the early stages of growth [15] to introduce corrective irrigation and alleviate stress. LWC is also useful for identifying plant genotypes that are tolerant to water stress and salinity by measuring the stability of LWC even under artificially induced water stress [18, 25]. Such experiments generally employ destructive procedures to obtain the LWC, which is time-consuming and labor intensive. Accordingly, this research has developed a non-destructive method to estimate LWC from UAV-based hyperspectral data.

==> Sections/3_Datasets.tex <==
\begin{figure*}[ht]
\vskip 0.1in
\begin{center}
\centerline{\includegraphics[width=17cm, height=4.5cm]{Images/ICML-Regression.pdf}}
\caption{LWC Prediction on Drone Hyperspectral Images: (a) Aerial Image of the Plot, (b) LWC Prediction for 20 Nov. 2018 (DAS=32), (c) LWC Prediction for 19 Dec. 2018 (DAS=63), (d) LWC Prediction on 10 Feb. 2019 (DAS=115).The color represents the range of water content and corresponds to the Legend (far right of the image).}
\label{fig:LWC}
\end{center}
\vskip -0.3in
\end{figure*}

The Spectroradiometer-based 400-1000 nm hyperspetral data was collected from an experimental farmland during 2018-19 post-monsoon season. The experimental farmland consists of plants grown in specialized treatment plots with varying levels of fertilizers and irrigation provided at regular intervals. There were 27 plots in total and the data collected includes hand-held and drone-based leaf-level hyperspectral signatures. Additionally, leaves were destructivly sampled from each treatment plots to obtain the ground-truth leaf water content using oven drying method.  The Spectroradiometer data were used to further analyze and estimate the leaf water content to ascertain the stress status. The resulting prediction model was then used to make a per-pixel stress prediction and water content estimation from the UAV Hyperspectral images of the entire plot captured during different crop growth stages. The Spectroradiometer data is used to predict stress and to estimate the leaf water content of the crop. The hyperspectral dataset consists of 483 data points from plants grown in specialized treatment plots with varying levels of fertilizers and irrigation. The dataset consists of 387 total columns including 382 Hyperspectral bands, DAS (Days After Sowing), Nitrogen, Carbon, CNRatio and Water content.

==> Sections/5_Results.tex <==
The proposed methodology as summarized in Figure \ref{fig:flowchart} was trained on the 2018-19 treatment plots. The evaluation Hyperspectral images are for the same crop captured at varying stages of growth and DAS (Days After Sowing). The LWC estimation using the GBM regressor is reliable since it has been trained on the entire dataset for all growth stages with the ground truth water content information. The results for the R2 and RMSE values for the GBM regressor showed high correlation. The resulting water content estimation can thus be used to predict the stress status of each plot to the granularity of leaf captured by the Hyperspectral camera. We also train the GBM classifier on only the 36 DAS data which includes only 78 data points to verify our hypothesis that computing LWC and then predicting Water Stress is more reliable. The low number of samples for DAS=36 is a limiting factor in the performance of using only the classification algorithm as opposed to using the LWC values to predict waterr stress. We found the Gradient Boosting Regressor to have the best performance metric for our predictions. We also identify the best fit parameters for the GBR using a rigorous hyperparameter search for the best set of parameters.


